Ecology, Spatial Structure, and Selection Pressure Induce Strong Signatures in Phylogenetic Structure

Evolutionary dynamics are shaped by a variety of fundamental, generic drivers, including spatial structure, ecology, and selection pressure. These drivers impact the trajectory of evolution, and have been hypothesized to influence phylogenetic structure. Here, we set out to assess (1) if spatial structure, ecology, and selection pressure leave detectable signatures in phylogenetic structure, (2) the extent, in particular, to which ecology can be detected and discerned in the presence of spatial structure, and (3) the extent to which these phylogenetic signatures generalize across evolutionary systems. To this end, we analyze phylogenies generated by manipulating spatial structure, ecology, and selection pressure within three computational models of varied scope and sophistication. We find that selection pressure, spatial structure, and ecology have characteristic effects on phylogenetic metrics, although these effects are complex and not always intuitive. Signatures have some consistency across systems when using equivalent taxonomic unit definitions (e.g., individual, genotype, species). Further, we find that sufficiently strong ecology can be detected in the presence of spatial structure. We also find that, while low-resolution phylogenetic reconstructions can bias some phylogenetic metrics, high-resolution reconstructions recapitulate them faithfully. Although our results suggest potential for evolutionary inference of spatial structure, ecology, and selection pressure through phylogenetic analysis, further methods development is needed to distinguish these drivers' phylometric signatures from each other and to appropriately normalize phylogenetic metrics. With such work, phylogenetic analysis could provide a versatile toolkit to study large-scale evolving populations.

==> Dockerfile <==
FROM mmore500/docker-texlive-full:sha-ea45eb5

COPY . /opt/hstrat-evolutionary-inference/tex

SHELL ["/bin/bash", "-c"]

# Define default working directory.
WORKDIR /opt/hstrat-evolutionary-inference/tex

# Prevent interactive time zone config.
# adapted from https://askubuntu.com/a/1013396
ENV DEBIAN_FRONTEND=noninteractive

RUN \
  echo 'Acquire::http::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::ftp::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::Retries "100";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo "buffed apt-get resiliency"

RUN \
  find /etc/apt -type f -name '*.list' -exec sed -i 's/\(^deb.*-backports.*\)/#\1/; s/\(^deb.*-updates.*\)/#\1/; s/\(^deb.*-proposed.*\)/#\1/; s/\(^deb.*-security.*\)/#\1/' {} + \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "removed -backports, -updates, -proposed, -security repositories"

# magic to fix java installation conflict in subsequent apt install
# see https://github.com/geerlingguy/ansible-role-java/issues/64
RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    man \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  mkdir /usr/share/man/man1/

RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    bibtool \
    ghostscript \
    git \
    make \
    moreutils \
    nodejs \
    pcregrep \
    pdftk \
    && \
  rm -rf /var/lib/apt/lists/*

CMD ["bash"]


==> Makefile <==
SHELL=/bin/bash

# get the basename of the containing directory
# this will be used to name othe output document
BUILD_DIR := $(shell basename $(abspath $(dir $(lastword $(MAKEFILE_LIST)))))

DRAFT_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}-draft.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

RELEASE_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

all: ${BUILD_DIR}-draft.pdf

draft: ${BUILD_DIR}-draft.pdf ${BUILD_DIR}-manuscript-draft.pdf ${BUILD_DIR}-supplement-draft.pdf ${BUILD_DIR}-draft.tex

release: ${BUILD_DIR}.pdf ${BUILD_DIR}-manuscript.pdf ${BUILD_DIR}-supplement.pdf ${BUILD_DIR}.tex

${BUILD_DIR}.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR} \
    -pdflatex="pdflatex -interaction=nonstopmode" main.tex

${BUILD_DIR}-distilled.pdf: ${BUILD_DIR}.pdf
	./script/rasterize-images.sh ${BUILD_DIR}.pdf ${BUILD_DIR}-distilled.pdf

${BUILD_DIR}.tex: main.tex
	./script/latexpand.pl main.tex > ${BUILD_DIR}.tex

${BUILD_DIR}-manuscript.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat 1-$$(( $(RELEASE_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript.pdf

${BUILD_DIR}-supplement.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat $(RELEASE_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement.pdf

${BUILD_DIR}-draft.pdf: main.tex
	latexmk -pdf -silent \
    --shell-escape \
    -jobname=${BUILD_DIR}-draft \
    -pdflatex="pdflatex -interaction=nonstopmode" draft.tex

${BUILD_DIR}-draft-distilled.pdf: ${BUILD_DIR}-draft.pdf
	./script/rasterize-images.sh ${BUILD_DIR}-draft.pdf ${BUILD_DIR}-draft-distilled.pdf

${BUILD_DIR}-draft.tex: main.tex
	./script/latexpand.pl draft.tex > ${BUILD_DIR}-draft.tex

${BUILD_DIR}-manuscript-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat 1-$$(( $(DRAFT_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript-draft.pdf

${BUILD_DIR}-supplement-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat $(DRAFT_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement-draft.pdf

fresh: cleaner all

clean:
	rm -f ${BUILD_DIR}.pdf
	rm -f ${BUILD_DIR}.tex
	rm -f ${BUILD_DIR}-draft.pdf
	rm -f ${BUILD_DIR}-draft.tex
	rm -f ${BUILD_DIR}-manuscript.pdf
	rm -f ${BUILD_DIR}-manuscript-draft.pdf
	rm -f ${BUILD_DIR}-supplement.pdf
	rm -f ${BUILD_DIR}-supplement-draft.pdf

sview:
	xdg-open ${BUILD_DIR}-draft.pdf 2>/dev/null

cleaner: clean
	latexmk -CA
	# remove auxillary files, excepting .tex and .bib files
	find . -type f -name ${BUILD_DIR}"*" ! -name '*.tex' ! -name '*.bib' -delete
	rm -rf *.bbl *.blg *.aux

.PHONY: draft release clean sview cleaner fresh


==> fig/perfect-tree-phylometrics-heatmap-avida-gen3sis.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/avida/teeplots/epoch=0+mut_distn=default+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{Avida.}
  \end{subfigure}
  \vspace{1cm}
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/avida/teeplots/epoch=0+mut_distn=default+spatial=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{Avida, with spatial structure.}
  \end{subfigure}
  \vspace{1cm}
  \begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/gen3sis/teeplots/epoch=0+mut_distn=default+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{gen3sis.}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/gen3sis/teeplots/epoch=0+mut_distn=default+spatial=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{gen3sis, with spatial barriers}
    \label{fig:perfect-tree-phylometrics-heatmap-avida-gen3sis}
  \end{subfigure}
  \caption{Heatmap of normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenetic records.}
  \label{fig:perfect-tree-phylometrics-heatmap-avida-gen3sis}
\end{figure*}


==> fig/perfect-tree-phylometrics-heatmap-avida.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \end{noindent}
  \caption{%
    Heatmap of normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenetic records.
    See Supplementary Figure \ref{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis} for results under sensitivity analysis conditions.
  }
  \label{fig:perfect-tree-phylometrics-heatmap}
\end{figure*}


==> fig/perfect-tree-phylometrics-heatmap-gen3sis.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=0.5\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \includegraphics[width=0.5\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+spatial=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \end{noindent}
  \caption{%
  \textbf{Phylometrics in Gen3sis.}
   Evolutionary regimes' effect sizes relative to ``plain'' baseline under the Gen3sis model with perfect phylogenetic tracking, normalized via Cliff's delta.
    Sample sizes $n=30$.
  }
\end{figure*}


==> fig/perfect-tree-phylometrics-heatmap.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \end{noindent}
  \caption{%
    Heatmap of normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenetic records.
    See Supplementary Figure \ref{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis} for results under sensitivity analysis conditions.
  }
  \label{fig:perfect-tree-phylometrics-heatmap}
\end{figure*}


==> fig/perfect-tree-phylometrics-parametric-heatmap.tex <==
\begin{figure*}
  \centering
\includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+normed=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
\caption{%
  Heatmap of normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenetic records.
  See Supplementary Figure \ref{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis} for results under sensitivity analysis conditions.
}
  \label{fig:perfect-tree-phylometrics-parametric-heatmap}
\end{figure*}


==> lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
  % adapted from https://tex.stackexchange.com/a/33577
  \ifdefined\DISSERTATION
  \else
    #1
  \fi
}


==> lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
  % adapted from https://tex.stackexchange.com/a/33577
  \ifdefined\DISSERTATION%
    #1%
  \else%
  \fi
  asdf
}


==> lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
\def\importpath{\import@path}
\makeatother


==> lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}

